Generating Equivalent Representations of Code By A Self-Reflection Approach

Equivalent Representations (ERs) of code are textual representations that preserve the same semantics as the code itself, e.g., natural language comments and pseudocode. ERs play a critical role in software development and maintenance. However, how to automatically generate ERs of code remains an open challenge. In this paper, we propose a self-reflection approach to generating ERs of code. It enables two Large Language Models (LLMs) to work mutually and produce an ER through a reflection process. Depending on whether constraints on ERs are applied, our approach generates ERs in both open and constrained settings. We conduct a empirical study to generate ERs in two settings and obtain eight findings. (1) Generating ERs in the open setting. In the open setting, we allow LLMs to represent code without any constraints, analyzing the resulting ERs and uncovering five key findings. These findings shed light on how LLMs comprehend syntactic structures, APIs, and numerical computations in code. (2) Generating ERs in the constrained setting. In the constrained setting, we impose constraints on ERs, such as natural language comments, pseudocode, and flowcharts. This allows our approach to address a range of software engineering tasks. Based on our experiments, we have three findings demonstrating that our approach can effectively generate ERs that adhere to specific constraints, thus supporting various software engineering tasks. (3) Future directions. We also discuss potential future research directions, such as deriving intermediate languages for code generation, exploring LLM-friendly requirement descriptions, and further supporting software engineering tasks. We believe that this paper will spark discussions in research communities and inspire many follow-up studies.

==> figure/listing_code_trans.tex <==
\begin{tcolorbox}[
            left=2pt, right=2pt, top=2pt, bottom=2pt,
            boxrule=0.2mm,
            arc=0mm,
            leftrule=2mm,
            colframe=black!40!white,
            colback=black!5!white,
            colbacktitle=black!50!white,
            colback=white]
Input Python Function:
\begin{lstlisting}[style=python]
import math
def compute_average(a, b):
    return math.floor((a + b) / 2.0)
\end{lstlisting}
    
Generated Java Method (The third trial):
\begin{lstlisting}[style=python]
import static java.lang.Math.floor;
public static int computeAverage(int a, int b) {
    return floor((a + b) / 2.0);
}
\end{lstlisting}

Generated Java Method (Final output):
\begin{lstlisting}[style=python]
import static java.lang.Math.floor;
public static int computeAverage(int a, int b) {
    return (int) floor((a + b) / 2.0);
}
\end{lstlisting}
\end{tcolorbox}

==> figure/listing_emoji.tex <==
\begin{tcolorbox}[
            left=2pt, right=2pt, top=2pt, bottom=2pt,
            boxrule=0.2mm,
            arc=0mm,
            leftrule=2mm,
            colframe=black!40!white,
            colback=black!5!white,
            colbacktitle=black!50!white,
            colback=white]
Input Code:
\begin{lstlisting}[style=python]
" ".join(content.split(" ")[:-1])
\end{lstlisting}
    
ER (Emoji):
\texttt{(" ")}\hspace{0.1em}\faLink\hspace{0.1em}\texttt{(content}\hspace{0.1em}\faCut\hspace{0.1em}\texttt{(" ")[}\faBan\hspace{0.1em}\texttt{end])}
\end{tcolorbox}

==> figure/listing_reflection.tex <==
\begin{tcolorbox}[
            left=2pt, right=2pt, top=2pt, bottom=2pt,
            boxrule=0.2mm,
            arc=0mm,
            leftrule=2mm,
            colframe=black!40!white,
            colback=black!5!white,
            colbacktitle=black!50!white,
            colback=white]
Input Code:
\begin{lstlisting}[style=python]
sum(sum(i) if isinstance(i, list) else i for i in L)
\end{lstlisting}
    
ER (1-th trial):
\begin{lstlisting}[style=python]
SUM(
  FOR EACH element i IN L:
    IF i IS A LIST:
      SUM(i)
    ELSE:
      i
)
\end{lstlisting}

ER (final output):
\begin{lstlisting}[style=python]
INITIALIZE total_sum TO 0
FOR EACH i IN L DO
    IF i IS INSTANCE OF list THEN
        total_sum = total_sum + SUM OF ELEMENTS IN i
    ELSE
        total_sum = total_sum + i
END FOR
RETURN total_sum
\end{lstlisting}
\end{tcolorbox}

==> figure/listing_table.tex <==
\begin{tcolorbox}[
            left=2pt, right=2pt, top=2pt, bottom=2pt,
            boxrule=0.2mm,
            arc=0mm,
            leftrule=2mm,
            colframe=black!40!white,
            colback=black!5!white,
            colbacktitle=black!50!white,
            colback=white]
Input Code:
\begin{lstlisting}[style=python]
self.driver.find_element_by_css_selector('.someclass a').get_attribute('href')
\end{lstlisting}
    
ER (Table):
\begin{lstlisting}[style=python]
| DriverContext  | Action | Selector  | Attribute |
|----------------|--------|---------- |-----------|
| self.driver    | Find   | '.someclass a' | href |
\end{lstlisting}
\end{tcolorbox}

==> figure/listing_xml.tex <==
\begin{tcolorbox}[
            left=2pt, right=2pt, top=2pt, bottom=2pt,
            boxrule=0.2mm,
            arc=0mm,
            leftrule=2mm,
            colframe=black!40!white,
            colback=black!5!white,
            colbacktitle=black!50!white,
            colback=white]
Input Code:
\begin{lstlisting}[style=python]
MyModel.objects.update(timestamp=F('timestamp') + timedelta(days=36524.25))
\end{lstlisting}
    
ER (XML):
\begin{lstlisting}[style=python]
<ObjMethod>
 <ClassName>MyModel</ClassName>
 <MethodName>objects.update</MethodName>
 <Assignment>
  <FieldName>timestamp</FieldName>
  <Expression>
   <FuncCall>
    <FuncName>F</FuncName>
    <Arg>timestamp</Arg>
    <Operator>+</Operator>
    <FuncCall>
     <FuncName>timedelta</FuncName>
     <KwArg>
      <Key>days</Key>
      <Value>36524.25</Value>
     </KwArg>
    </FuncCall>
   </FuncCall>
  </Expression>
 </Assignment>
</ObjMethod>
\end{lstlisting}
\end{tcolorbox}
